The Vickrey Auction with a Single Duplicate Bidder Approximates the Optimal Revenue

Bulow and Klemperer's well-known result states that, in a single-item auction where the $n$ bidders' values are independently and identically drawn from a regular distribution, the Vickrey auction with one additional bidder (a duplicate) extracts at least as much revenue as the optimal auction without the duplicate. Hartline and Roughgarden, in their influential 2009 paper, removed the requirement that the distributions be identical, at the cost of allowing the Vickrey auction to recruit $n$ duplicates, one from each distribution, and relaxing its revenue advantage to a $2$-approximation. In this work we restore Bulow and Klemperer's number of duplicates in Hartline and Roughgarden's more general setting with a worse approximation ratio. We show that recruiting a duplicate from one of the distributions suffices for the Vickrey auction to $10$-approximate the optimal revenue. We also show that in a $k$-items unit demand auction, recruiting $k$ duplicates suffices for the VCG auction to $O(1)$-approximate the optimal revenue. As another result, we tighten the analysis for Hartline and Roughgarden's Vickrey auction with $n$ duplicates for the case with two bidders in the auction. We show that in this case the Vickrey auction with two duplicates obtains at least $3/4$ of the optimal revenue. This is tight by meeting a lower bound by Hartline and Roughgarden. En route, we obtain a transparent analysis of their $2$-approximation for $n$~bidders, via a natural connection to Ronen's lookahead auction.

==> app-k-item-free-backup.tex <==
\begin{theorem}
\TheoremName{kUnitFree}
In a $k$-item auction with $n$ bidders whose values are drawn independently from (non-identical)
regular distributions $F_1, \ldots, F_n$, there exists $i$ such that the second price auction
with the same $n$ bidders and additional bidders $n+1, \ldots, n+k$ whose values are drawn independently
from $F_i$ achieves at least $0.0008$ fraction of the ex ante optimal revenue with the original $n$ bidders.
\end{theorem}
\begin{proof}
We will consider the three cases of \Lemma{kItemsCases}.

\paragraph{Case 1: There exists $i_1, \ldots, i_r$ where $r \leq k$ such that $\sum_{j=1}^{r} \val_{i_j}(\beta) \geq \delta \OPT$.}
By shuffling around the indices, let us assume that these bidders are $1, \ldots, r$.
Note that we also have $\val_i(\beta) \geq \frac{\gamma}{k} \OPT$.
Moreover, this case implies that $\sum_{i=1}^r \Rev_i(\beta) \geq \beta \delta \OPT$.

The next step is to partition the bidders into different ``levels'' corresponding to how large their values are at a quantile of $\beta$.
Specifically, for $t \geq 1$ define the set $S_t = \{ i \in [r] : \Rev_i(\beta) \in \OPT \cdot (2^{-t}, 2^{-t+1}] \}$.
Let $T = \lg\left( \frac{k}{\gamma} \right)$.
By definition of $r$, $S_t = \emptyset$ for all $t > T$.
Finally, define $h = \min\{t : S_t \neq \emptyset\}$.
We will consider two subcases based on the value of $h$.
\paragraph{Case 1a: $h < 6 - \lg\left( 31 \beta \delta - 2\gamma \right)$.}
In this case, there is already a bidder with fairly large value.
In particular, there must exist a bidder $i$ such that $\Rev_i(\beta) \geq \frac{\OPT}{2^h} = \frac{3 \beta \delta \OPT}{25}$.
By \Claim{reg}, this implies that $\Rev_i(1 - 1/k) \geq \frac{3 \beta \delta \OPT}{25k}$.
This implies that $\val_i(1-1/k) \geq \frac{3 \beta \delta \OPT}{25k}$ as well.
Now suppose that we duplicate this bidder $i$ a total of $k$ times.
The probability that one of these bidders bid at least $\frac{3 \beta \delta \OPT}{25k}$ is at least $1 - 1/k$.
Hence, the probability that all $k+1$ copies of bidder $i$ bid above $\frac{3\beta \delta \OPT}{25k}$ is at least $(1-1/k)^{k+1}$.
Since $k \geq 2$, the latter quantity is at least $1/8$.
We conclude that, in this case, the revenue of SPA with the $k$ duplicates is at least $\frac{3 \beta \delta \OPT}{200}$.

\paragraph{Case 1b: $h \geq 6 - \lg \left( 31 \beta \delta - 2\gamma \right)$.}
This case is a bit more technical because the bidders may be ``spread out'' amongst the different levels.
Nonetheless, we claim that duplicating a bidder in $S_h$ will allow SPA to extract a constant fraction of the ex-ante revenue.

Let $n_t = |S_t|$.
By definition of $S_t$, we have the inequality
\[
    \beta \delta \OPT
    \leq
    \sum_{i=1}^r \Rev_i(\beta)
    = \sum_{t=1}^{T} \sum_{i \in S_t} \Rev_i(\beta)
    \leq 2 \sum_{t=1}^T n_t 2^{-t} \OPT.
\]
In particular, this asserts that
\begin{equation}
    \EquationName{weird}
    \sum_{t=1}^T n_t 2^{-t} \geq \frac{\beta \delta}{2}.
\end{equation}
This inequality will be useful for us in a few moments.

Let $i \in S_t$.
Then by definition, we have $\Rev_i(\beta) \geq \OPT / 2^t$.
Hence, \Claim{reg} implies that $\Rev_i\left( 1 - \frac{2^t \gamma}{32k} \right) \geq \frac{\gamma \OPT}{32k}$.
In particular, $\val_i\left(1 - \frac{2^t \gamma}{32k} \right) \geq \frac{\gamma \OPT}{32k}$.
As stated above, we can duplicate any bidder in $S_h$ exactly $k$ times.

Let $S$ be the number of bidders that bid at least $\frac{\gamma \OPT}{32k}$ amongst the original $r$ bidders and the $k$ duplicates.
Then we have
\begin{align*}
    \Ex S
    & \geq
    k \left( 1 - \frac{2^h \gamma}{32k} \right) + \sum_{t=h}^{T} n_t \left( 1 - \frac{2^t \gamma}{32k} \right) \\
    & =
    k \left( 1 - \frac{2^h \gamma}{32k} \right) + \sum_{t=h}^{T} n_t 2^{-t} 2^{t} \left( 1 - \frac{2^t \gamma}{32k} \right) \\
    & \geq
    k \left( 1 - \frac{2^h \gamma }{32k} \right) + 2^h\sum_{t=h}^{T} n_t 2^{-t} \left( 1 - \frac{2^t \gamma}{32k} \right) \\
    & \geq
    k \left( 1 - \frac{2^h \gamma }{32k} \right) + 2^h \cdot \frac{31}{32} \sum_{t=h}^{T} n_t 2^{-t} \\
    & \geq
    k \left( 1 - \frac{2^h \gamma }{32k} \right) + 2^h \cdot \frac{31 \beta \delta }{64} \\
    & =
    k + 2^{h} \beta \delta \left( \frac{31 \beta \delta }{64} - \frac{2\gamma}{64} \right) \\
    & \geq
    k + \frac{32}{3} \left( \frac{15}{64} - \frac{1}{32} \right) \\
    & \geq k + 2,
\end{align*}
where the second inequality uses the bound $2^t \geq 2^h$,
the third inequality uses that $T = \lg\left( \frac{k}{\gamma} \right)$ so $1 - \frac{2^T \beta \delta}{32k} \geq \frac{31}{32}$,
the fourth inequality uses \Equation{weird}, and the fifth inequality uses the assumption that $h \geq 6 - \lg \left( 31 \beta \delta - 2 \gamma \right)$.
Now observe that $N$ is a sum of independent Bernoulli random variables, albeit with random means.
Combining \Theorem{Hoeffding} and \Fact{median}, we conclude that at least $k + 1$ bidders bid at least $\frac{\beta \delta \OPT}{32k}$
with probability at least $1/2$.
Hence, in this case SPA obtains a revenue of at least $\frac{\gamma \OPT}{64}$.

\paragraph{Case 2: There exist $k$ bidders $i_1, \ldots, i_k$ who each bid at least $\frac{\gamma}{k} \OPT$ with probability at least $\beta$.}
By renaming the bidders, suppose that bidders $1, \ldots, k$ each bid at least $\frac{\gamma}{k} \OPT$ with probability at least $\beta$,
i.e.~$\val_i(\beta) \geq \frac{\gamma}{k} \OPT$ for $i \in [k]$.
Moreover, we can also write $\Rev_i(\beta) \geq \frac{\beta \gamma}{k} \OPT$.
By \Claim{reg}, we have $\Rev_i(3/4) \geq \frac{\beta \gamma}{4k} \OPT$, so $\val_i(3/4) \geq \frac{\beta \gamma}{3k} \OPT$.
We now obtain $k$ duplicates of bidder $1$.
Since we have $2k$ bidders in total and each bidder has probability $3/4$ of bidding at least $\frac{\beta \gamma}{3k} \OPT$,
we can apply \Theorem{Hoeffding} and \Fact{median} to assert that the probability that there are at least $3k/2 \geq k+1$ bidders that bid
at least $\frac{\beta \gamma}{3k} \OPT$ is at least $1/2$.
Hence, the revenue in this case is $\frac{\beta \gamma}{6} \OPT$.

\paragraph{Case 3: With probability at least $1 - \exp(-\frac{7}{512} \sqrt{k} )$ there exists at least $k + 1$ bidders who bid at least $\frac{\gamma}{k} \OPT$.}
This case is trivial by assumption.

Putting all our cases together, we get the revenue of SPA with $k$ duplicates is at least
\[
    \min\left\{ \frac{3 \beta \delta}{200}, \frac{\beta \delta}{64}, \frac{\beta \gamma}{6}, \left( 1 - \exp(-\frac{7}{512} \sqrt{k}) \right) \gamma \right\}.
\]
Plugging in $\beta = 2/3$, $\gamma = 4/33$, and $\delta = 8/99$ gives the stated bound.
\end{proof}

Let $\Ber(p)$ denote the Bernoulli distribution with mean $p$ and $\Binom(n,p)$ be the binomial distribution.
\begin{theorem}[Theorem~4 in \cite{Hoeffding56}]
\TheoremName{Hoeffding}
Let $X_1, \ldots, X_n$ be random variables where $X_i \sim \Ber(p_i)$.
Let $S = \sum_{i=1}^n X_i$ and set $p = n^{-1} \Ex S$.
Then for all $t \leq np - 1$, $\Pr[S \leq c] \leq \Pr[\Binom(n, p) \leq c]$.
\end{theorem}
\begin{fact}[Corollary~1 in \cite{KB80}]
\FactName{median}
The median of $\Binom(n,p)$ is at least $\lfloor np \rfloor$.
\end{fact}


==> app-k-item-free.tex <==
We begin with a technical lemma for $k$-item auctions with $n$ bidders.
\chris{This is a cleaned up lemma for the k item case and works for both the free setting and the constrained setting.
    In fact, it gives better results for both!}


Let $\Ber(p)$ denote the Bernoulli distribution with mean $p$ and $\Binom(n,p)$ be the binomial distribution.
\begin{theorem}[Theorem~4 in \cite{Hoeffding56}]
\TheoremName{Hoeffding}
Let $X_1, \ldots, X_n$ be random variables where $X_i \sim \Ber(p_i)$.
Let $S = \sum_{i=1}^n X_i$ and set $p = n^{-1} \Ex S$.
Then for all $t \leq np - 1$, $\Pr[S \leq c] \leq \Pr[\Binom(n, p) \leq c]$.
\end{theorem}
\begin{fact}[Corollary~1 in \cite{KB80}]
\FactName{median}
The median of $\Binom(n,p)$ is at least $\lfloor np \rfloor$.
\end{fact}
Let $X_1, \ldots, X_n$ be random variables where $X_i \sim \Ber(p_i)$, $S = \sum_{i=1}^n X_i$,a nd $p = n^{-1} \Ex S$.
Since $np - 1 \leq \lfloor np \floor$, \Theorem{Hoeffding} and \Fact{median} imply that
\[
    \prob{S \leq np-1} \leq \prob{S < \lfloor np \floor} \leq 1/2.
\]
Hence, $\prob{S \geq np} \geq 1/2$.


==> app-lookahead.tex <==
\begin{proof}[Proof of Lemma~\ref{lem:spa-lookahead}.]
% We analyze the following auction, whose revenue is clearly upper bounded by that of the second price auction with $n$ duplicate bidders:

	We say bidder~$n+i$ is bidder~$i$'s duplicate.  We will show that SPALD has a revenue no less than~$\LA$.  Let us condition on the realization of $\vali[1], \ldots, \vali[i^* - 1], \vali[i^* + 1], \ldots, \vali[n]$ (which henceforth we denote as $\vals_{[n] - i^*}$), and denote by $\sechigh$ the highest among them.  
% on the fact that $\vali[i^*]$ is higher than all of them.  
We show that, conditioning on this, the lookahead auction (without duplicates) obtains no more revenue from bidder~$i^*$ than SPALD does from bidder~$i^*$ \emph{and} her duplicate, bidder $n + i^*$.

% Let $\res_{i^*}$ be the monopoly reserve price of bidder~$i^*$.  
% \hufu{Define monopoly reserve in the prelim.}  
We first analyze the posted price faced by $i^*$ in the lookahead auction.  Recall that the lookahead auction posts the revenue-optimal price for $i^*$ conditioning on $\vali[i^*] \geq \sechigh$.
%
Conditioning on $\vali[i^*] \geq \sechigh$, the revenue by posting any price $p \geq \sechigh$ to bidder~$i^*$ is $p(1 - F_{i^*}(p)) / (1 - F_{i^*}(\sechigh))$, which is simply the unconditioned revenue at that price $p (1 - F_{i^*}(p))$ amplified by a constant factor $1 / (1 - F_{i^*}(p))$.   Therefore the shape of the revenue curve conditioned on $\vali[i^*] \geq \sechigh$ is simply bidder $i^*$'s revenue curve to the left of $q(\sechigh)$ and amplified by a constant factor.  Since the original revenue curve is concave, it is nondecreasing to the left of~$q_{i^*}(\monres_{i^*})$, the quantile of the monopoly reserve price, and non-increasing to the right.  Therefore, if $\sechigh$ is higher than $\monres_{i^*}$, 
% the monopoly reserve price for bidder~$i^*$, 
the lookahead auction will simply post $\sechigh$ as the take-it-or-leave-it price for bidder~$i^*$; otherwise, the lookahead auction uses $\monres_{i^*}$ as the price.\footnote{This analysis essentially shows that the lookahead acution in our setting is the second price auction with monopoly reserve prices.}

If $\sechigh \geq \monres_{i^*}$, the lookahead auction extracts $\sechigh$ from bidder~$i^*$ when $\vali[i^*] \geq \sechigh$; but whenever $\vali[i^*] \geq \sechigh$, SPALD extracts a revenue at least $\sechigh$ from bidders $i^*$ and $n + i^*$.

The case where $\sechigh < \monres_{i^*}$ needs more calculation.  Let $R_{i^*}$ be the monopoly revenue extractable from bidder~$i^*$ (i.e., $\monres_{i^*}(1 - F_{i^*}(\monres_{i^*})$).  The lookahead auction, by posting the monopoly reserve price $\monres_{i^*}$, extracts revenue $R_{i^*}$ from bidder~$i^*$.  
% \hufu{Define $q_i$ as a function in the prelim.} 
We show that SPALD gets at least as much from bidder~$i^*$ and her duplicate.  

% Since the duplicate bidder's value $\vali[n + i^*]$ is drawn from the same distribution $F_{i^*}$, the quantile of $\vali[n+i^*]$ is uniformly distributed between $0$ and~$1$ on the revenue curve of~$i^*$.  
Recall that the duplicate bidder's value $\vali[n + i^*]$ is drawn from the same distribution $F_{i^*}$ as bidder~$i^*$.
%
With probability $F_{i^*}(\sechigh)$, $\vali[n + i^*]$ is no more than~$\sechigh$, and SPALD extracts a revenue of $\Rev_{i^*}(q_{i^*}(\sechigh))$ from bidder~$i^*$.  When $\vali[n+ i^*] \geq \sechigh$, bidder~$i^*$ faces in SPALD a take-it-or-leave-it price of $\vali[n + i^*]$, and the expected revenue from bidder~$i^*$is precisely the height of $\Rev_{i^*}$ at the quantile of~$\vali[n+i^*]$.
Since $\vali[n+ i^*]$ is drawn from the same distribution, its quantile in $F_{i^*}$, namely, $q_{i^*}(\vali[n + i^*]) = 1 - F_{i^*}(\vali[n + i^*])$, is uniformly distributed on $[0, 1]$.  Therefore the expected revenue when $\vali[n + i^*] \geq \sechigh$ is 
% Since this quantile is uniform, this revenue in expectation is 
simply the area under bidder~$i^*$'s revenue curve between $0$ and~$q_{i^*}(\sechigh)$.
(See Figure~\ref{fig:rev-curve} for an illustration.\footnote{This conversion from the expected revenue to an area under the revenue curve is an elegant technique from \citet{DRY15}.}) 
%
The expected revenue from the duplicate bidder~$n + i^*$ is the same area: when $\vali[i^*]$ is at least~$\sechigh$, bidder~$n + i^*$ faces a take-it-or-leave-it price of $\vali[i^*]$, whose quantile in $F_{n + i^*}$ is uniform between $0$ and~$q_{n+i^*}(\sechigh)$, and therefore the expected revenue from bidder~$n+i^*$ is exactly the area under the revenue curve~$\Rev_{i^*}$ between quantiles $0$ and~$q_{i^*}(\sechigh)$.

Summing up the parts, the revenue of SPALD from bidders $i^*$ and~$n + i^*$ when $\sechigh \leq \monres_{i^*}$ is twice the area under the revenue curve $\Rev_{i^*}$ between $0$ and~$q_{i^*}(\sechigh)$,
plus the area of a rectangle with height $\Rev_{i^*}(q_{i^*}(\sechigh))$ and width $1 - q_{i^*}(\sechigh)$.  
%
If one replaces the part of the revenue curve $\Rev_{i^*}$ between $q_{i^*}(\monres_{i^*})$ and~$1$ by a straight line, the resulting curve is still concave, with the highest value at~$R_{i^*}$.  
%
Twice the area under this new curve is precisely SPALD's revenue from $i^*$ and~$n + i^*$.  By the concavity of the curve, this is still at least $R_{i^*}$.  This completes the proof.
\begin{figure}
\centering
\begin{tikzpicture}
\fill [fill = gray!30] (0, 0) -- (3, 0) -- (3, 1.166) -- (1, 3.5) -- cycle;
\draw [thick, ->] (0, 0) -- (5, 0) node[anchor = north west] {$q$};
\draw [thick, ->] (0, 0) -- (0, 4) node[anchor = south east] {$\Rev$};
\draw [thick] (0, 0) node[below]{$1$}  -- (1, 3.5) -- (4, 0) node[below] {$0$};
\draw [dashed] (1, 0) node[below]{$q(\monres)$} -- (1, 3.5);
\draw [dashed] (3, 0) node[below]{$q(\sechigh)$} -- (3, 1.166);
\end{tikzpicture}
\caption{Illustration of a concave revenue curve.  In this figure $\sechigh < \monres$, and the shaded area is the expected revenue from this bidder when both she and her duplicate bidder bid above $\sechigh$.}
\label{fig:rev-curve}
\end{figure}

\end{proof}



==> app-robust.tex <==
\chris{\Claim{reg_delta2} is new and fixes a previously faulty version of the claim.}
\chris{\textbf{TODO} Ensure \Claim{reg_delta2} is referenced and that the assumption that $q \in [0,1/2]$ is used.}

\begin{claim}
\ClaimName{reg_delta2}
Let $q \in [0,1/2]$ and $q' \in [0,1]$ be such that $|q - q'| \leq \eps q$ for some $\eps \in [0,1]$.
Then $(1-\eps) \Rev(q) \leq \Rev(q') \leq \frac{1}{1-\eps} \Rev(q)$.
\end{claim}
\begin{proof}
First suppose that $q' > q$.
By concavity of the revenue curve, we have
\begin{align*}
\Rev(q') & \geq \frac{1 - q'}{1-q} \Rev(q) + \frac{q - q'}{1-q} \Rev(1) \\
& \geq \frac{1-q'}{1-q} \Rev(q) \\
& \geq \frac{1-q+q-q'}{1-q} \Rev(q) \\
& = \left( 1 - \frac{q' - q}{1-q} \right) \Rev(q).
\end{align*}
Since $q \leq 1/2$, we have $q \leq 1 - q$.
So
\begin{align*}
    \Rev(q')
    & \geq \left( 1 - \frac{q' - q}{1-q} \right) \Rev(q) \\
    & \geq \left( 1 - \frac{\eps q}{1-q} \right) \Rev(q) \\
    & \geq \left( 1 - \frac{\eps (1-q)}{1-q} \right) \Rev(q) \\
    & = (1-\eps) \Rev(q).
\end{align*}
This proves the lower bound on $\Rev(q')$.
To get the upper bound, we use concavity again and note that
\begin{align*}
    \Rev(q)
    & \geq \frac{q}{q'} \Rev(q') + \frac{q'-q}{q} \Rev(0) \\
    & \geq \frac{q}{q'} \Rev(q') \\
    & \geq \frac{q' - \eps q}{q'} \Rev(q') \\
    & = (1 - \eps q / q') \Rev(q') \\
    & \geq (1-\eps) \Rev(q'),
\end{align*}
where the last inequality is because $q < q'$.
So $\Rev(q') \leq \frac{1}{1-\eps} \Rev(q')$.

The case of $q' < q$ follows from calculations which are similar to those above.
Indeed
\begin{align*}
\Rev(q') & \geq \frac{q'}{q} \Rev(q) + \frac{q-q'}{q} \Rev(0) \\
& \geq \frac{q'}{q} \Rev(q) \\
& \geq \frac{(1-\eps)}{q} \Rev(q) \\
& \geq (1-\eps)\Rev(q)
\end{align*}
and
\[
\Rev(q)
\geq \left( 1 - \frac{q - q'}{1-q'} \Rev(q') \right).
\]
Since $q' < q \leq 1/2$, we have $q \leq 1 - q \leq 1 - q'$.
So $q - q' \leq \eps q \leq \eps(1-q')$ and this shows that $\Rev(q) \geq (1-\eps) \Rev(q')$ as desired.
\end{proof}


==> app-single-item.tex <==
\begin{claim}
\ClaimName{reg}
Suppose that $0 \leq q \leq q' \leq \beta \leq 1$.
Then for any regular distribution, we have $\Rev(q') \geq (1 - \beta) \Rev(q)$.
\end{claim}
\begin{proof}
By the concavity of the revenue curves, we have
\[
    \Rev(q') \geq \frac{1-q'}{1-q} \Rev(q) + \frac{q'-q}{1-q} \Rev(1) \geq (1-\beta) \Rev(q),
\]
since $\Rev(1) \geq 0$.
\end{proof}

